LADICA: A Large Shared Display Interface for Generative AI Cognitive Assistance in Co-Located Team Collaboration

Large shared displays, such as digital whiteboards, are useful for supporting co-located team collaborations by helping members perform cognitive tasks such as brainstorming, organizing ideas, and making comparisons. While recent advancement in Large Language Models (LLMs) has catalyzed AI support for these displays, most existing systems either only offer limited capabilities or diminish human control, neglecting the potential benefits of natural group dynamics. Our formative study identified cognitive challenges teams encounter, such as diverse ideation, knowledge sharing, mutual awareness, idea organization, and synchronization of live discussions with the external workspace. In response, we introduce LADICA, a large shared display interface that helps collaborative teams brainstorm, organize, and analyze ideas through multiple analytical lenses, while fostering mutual awareness of ideas and concepts. Furthermore, LADICA facilitates the real-time extraction of key information from verbal discussions and identifies relevant entities. A lab study confirmed LADICA's usability and usefulness.

==> paper/Design_Goal.tex <==
\section{Design goals}

Based on our formative study findings and theories on the cognitive processes of team collaboration introduced in Section \ref{sec:cognition_theory}, we have identified four design goals for an LLM-enhanced large shared display interface to facilitate co-located team collaboration. 
% We first describe the design goals and then present a scenario to illustrate how these goals can be realized through our system.

\paragraph{\textbf{DG1: Enhancing dynamic ideation and knowledge sharing within groups}}

Social and motivational barriers, such as fear of being judged negatively and social loafing, can prevent team members from freely sharing their ideas and knowledge, thus affecting the inclusivity and richness of team interactions. Moreover, cognitive theories and insights from our formative study emphasize the importance of metacognitive support. This type of support aids teams in recognizing the structure of complex, abstract tasks. Besides, team members often need help articulating and refining their ideas during frequent discussions and recognizing relevant ideas that may otherwise be overlooked. To address these challenges, our proposed system aims to provide cognitive assistance to support these dynamic ideation processes and promote knowledge sharing.


% In-person team collaboration can be hindered by social-motivational factors such as the fear of negative evaluation and social loafing, which may deter members from sharing their ideas and knowledge and reduce the inclusiveness of team participation. In addition, both cognitive theories and our formative study indicate that it is beneficial to provide a meta-cognition support that help team recognize the structure of the abstract tasks they are addressing. Moreover, individuals often need to delve into articulating and expanding their ideas during frequent discussions and pay attention to relevant ideas they might overlook. Therefore, our system should offer cognitive assistance to support these dynamic ideation processes and promote knowledge sharing.
% In addition, effective collaboration often requires the team to explore various approaches to decompose and delegate team tasks, and think both broadly and deeply about the topics they are addressing. In response, our proposed system should encourage the knowledge contribution from each member and inspire their ideation process.

\paragraph{\textbf{DG2: Fostering collaborative cues without overriding human interaction}}

% make it strong, do not want to overley on AI, AI intervention effect on existing human-human collaboration

% over-scripting: too much support will hurt collaboration

The ability to maintain mutual awareness is essential to identify collaborative opportunities, especially when team members work on different tasks in parallel. The results of our formative study underline the difficulties in achieving and preserving this awareness, often due to cognitive overload. While participants are open to AI assistance for better cognitive processing, there is a concern that too much AI involvement could overpower natural team dynamics and hinder direct interactions among team members. Thus, our system is designed to help teams understand how their contributions are interconnected, enhancing collaboration cues. At the same time, it aims to avoid overtaking the collaboration process. The design should refrain from automatically completing group tasks that demand group discussion or excessively controlling the discussion flow or prescribing the sequence of topic discussion.

\paragraph{\textbf{DG3: Enabling diverse and comprehensive perspectives in analyzing shared content}}

Our formative study highlighted the need for teams to analyze and group ideas from a variety of analytical perspectives to uncover themes or connections. However, this process can be challenging and demanding as it involves selecting the right perspectives and organizing ideas accordingly. Additionally, it is essential for teams to track the evolution of these patterns and relationships as collaboration progresses. Lastly, team members require a function for saving and reloading workspace snapshots so that they can freely experiment with different grouping results and revert to a previous version if desired.  To address these needs, our system should facilitate the grouping analysis from different perspectives, aiding teams in both the creation and the discussion phases. 


% Our formative study revealed that users need to conduct grouping analysis of group ideas from various analytical perspectives to identify common affinities or themes. However, determining the appropriate perspectives and grouping ideas accordingly can be time-consuming and mentally taxing. In addition, teams must keep track of how these patterns and relationships develop as collaboration progresses. Therefore, our system should support teams in conducting and monitoring the results of grouping from different perspectives during team creation and discussion.

% Our participants indicated that in co-located teamwork, conducting meta-analyses on whiteboards, such as dimensional and relational analysis, can be challenging and time-consuming due to visual clutter. These analyses are crucial for teams to identify patterns, relationships, and key themes. Furthermore, teams need to monitor how these patterns and relationships evolve as collaboration progresses. Therefore, our system should facilitate and support groups in performing and auditing various types of meta-analyses.


\paragraph{\textbf{DG4: Streamlining discussion and workspace synchronization}}

Co-located group collaboration often includes a significant amount of informal discussion. Our formative study identified a challenge: synchronizing these dynamic discussions with the representation in the group shared space can be cognitively demanding. There is a need for a system that can identify and bring forward crucial points from discussions, highlighting relevant information already present in the workspace. By doing so, our system aims to bridge the gap between verbal exchanges and visual representations, ensuring that key discussion elements are effectively integrated into the collaborative workspace.


==> paper/Scenario.tex <==
\section{Example Scenario}

==> paper/archive/Introduction.tex <==
\section{INTRODUCTION}

\textit{Collocated interaction}, where team members share a physical space and communicate face-to-face, remains a pervasive and irreplacable team workstyle in digital era~\cite{olson2000distance, olsson2020technologies}. This ``same time, same place'' form of interaction provides numerous benefits, including instant feedback between participants, non-verbal cues, and a common physical setting that is shared among all those present. Compared to remote collaboration, collocated interaction is said to be advantageous in promoting deeper conversations~\cite{bagheri2021comparative, ellis2006and}, encouraging collective creativity and productivity~\cite{olson2000distance}, and nurturing a sense of belonging and connection~\cite{caplan2002problematic, sacco2014social, liu2022understanding} among group members. 

% Single groupware display 
Given the unique advantages of this setting, the HCI professionals have consistently worked on designing groupware systems that enhance support for collocated interactions. Among the prevalent systems in this domain is Single Display Groupware (SDG)~\cite{stewart1999single}, which supports a group of members to work together on a large, shared interactive screen. Compared with multi-display setup, SDG empowers participants to display and structure information within a co-present scaled workspace, enhance their mutual understanding using a shared local context~\cite{luck2013visual, risko2016cognitive}, and augment their engagement not only through verbal dialogue but also through nonverbal cooperative gestures~\cite{liu2017coreach}. In designing SDG, a primary design goal of prior works is to accommodate dynamic collaboration patterns between coworkers. As Olson et al.~\cite{olson2000distance} suggests, collaborative works often need varied degrees of \textit{coupling}\footnote{Coupling is defined as the frequency of interaction among team members relative to the volume of tasks that need to be completed}. For complex tasks such as planning and sensemaking, there are often ambiguous and non-routine aspects that demand closely coordinated efforts with regular communication. Conversely, the more routine aspects of team activities are typically segmented into individual tasks so that members can execute concurrently. 

Following Gutwin's identified three desiderata about groupware for dynamic collaboration~\cite{gutwin1998design}, many prior works in SDG have innovated techniques for workspace navigation \hl{[...]}, artifact manipulation ~\cite{liu2016shared, liu2017coreach}, and view representation \hl{[...]} to balance the needs of group and individual works on a same screen. While these studies offer insights into improving the functionality and accessibility of SDG, their primary emphasis has been on enhancing the aspects of manipulation and visualization. However, there is still a lack of exploration in how to design SDGs to offer in-situ scaffolding for collaborative tasks that demand high coordination costs, such as group decision-making, planning, and argumentation. At the group level, those tasks require individuals to negotiate or build consensus with each other alternating between group and individual work, which needs people to frequently switch working memory and apply various communication skills. On the other hand, as individuals process work, they may go through multiple phases such as brainstorming, planning, and prototyping. In the meantime, they need to maintain a mutual awareness of potential collaboration opportunities or conflicts. The inability to adequately address these requirements and the diverse capabilities of individuals can lead to problems like social loafing and misalignment within the group.

\hl{Current Foundation Model limitation}

% Prior works have presented SDG for supporting a variety of group tasks such as collaborative sensemaking~\cite{shi2017ideawall}, searching~\cite{ruddle2015performance}, and exploratory visual analysis~\cite{reda2015effects}. 



% A large, multi-touch display is a common interactive device used for collocated interaction. Compared with physical mediums such as "post-it" notes, a large digital display offers enhanced flexibility for social interaction and spatial organization within a scalable space, along with seamless integration with various digital support tools~\cite{olsson2020technologies}. As a shared workspace, this kind of interactive display maintains group awareness of the current task~\cite{olson2000distance}. Besides, those displays could visualize and externalize the working memory to offload and scaffold group thinking~\cite{luck2013visual, risko2016cognitive}, and the shared concept mapping could reduce communication ambiguities and information distortion~\cite{kraut2002use, dimicco2004influencing}. Given those favorable characteristics, prior works have focused on designing and developing large display-based interfaces to \hl{enable novel gestural interaction and visualization}. For example, Dynamo~\cite{izadi2003dynamo} uses a public interactive surface to support the cooperative sharing and exchange of media. CoReach~\cite{liu2017coreach} enables a set of cooperative gestures that combines multiple users’ multi-touch gestural input to trigger actions for passing or showing content to each other. IdeaWall~\cite{shi2017ideawall} continuously extracts essential information from a verbal discussion and augments that information with web-search materials on display. 

% Though most prior works aim at facilitating collocated tasks at the interaction level,  individuals may encounter various cognitive and social-motivational challenges beyond interaction~\cite{ez2023group}. Prior studies found that co-presenting people are prone to being trapped in issues such as evaluation apprehension, social loafing, and misalignment of mental states. Moreover, tasks, such as group brainstorming and decision-making, demand participants to adapt to dynamic work styles, including both synchronous and parallel cooperation. These tasks also require engaging in various forms of social interaction, like argumentation and consensus-building, which call for a mix of individual and collective reasoning activities. So far, it is still under-explored that \textit{how can a large display interface be designed to provide cognitive and social-motivational support for both individual and group work in a collocated setting?}

In this work, we first conducted a literature review to understand (1) common cognitive and social-motivational challenges in collocated interaction, (2) existing design approaches to dealing with those challenges, and (3) the design gaps of existing shared displays. Based on these lessons, we then conducted a design workshop with \hl{xx} students to brainstorm and concertize the design goals that our large display application should achieve.


